Lower Bounds for Approximating Graph Parameters via Communication Complexity

In a celebrated work, Blais, Brody, and Matulef developed a technique for proving property testing lower bounds via reductions from communication complexity. Their work focused on testing properties of functions, and yielded new lower bounds as well as simplified analyses of known lower bounds. Here, we take a further step in generalizing the methodology of Blais et al. to analyze the query complexity of graph parameter estimation problems. In particular, our technique decouples the lower bound arguments from the representation of the graph, allowing it to work with any query type. We illustrate our technique by providing new simpler proofs of previously known tight lower bounds for the query complexity of several graph problems: estimating the number of edges in a graph, sampling edges from an almost-uniform distribution, estimating the number of triangles (and more generally, $r$-cliques) in a graph, and estimating the moments of the degree distribution of a graph. We also prove new lower bounds for estimating the edge connectivity of a graph and estimating the number of instances of any fixed subgraph in a graph. We show that the lower bounds for estimating the number of triangles and edge connectivity also hold in a strictly stronger computational model that allows access to uniformly random edge samples.

==> counting-edges.tex <==
%% \DeclareMathOperator{\neighbor}{nbr}
%% \DeclareMathOperator{\degree}{deg}
%% \DecoareMathOperator{\pair}{pair}

\subsection{Counting and Sampling Edges}

% Recall results of Goldreich and Ron, also Feige

\subsubsection{Counting Edges}
\label{sec:counting-edges}

We start by proving a result of~\cite{Goldreich2008} that gives
a lower bound of $\Omega(n/\sqrt{\e m})$ for estimating the number of edges in a graph up to a $(1\pm \e/2)$-multiplicative factor using degree, neighbor and pair queries. A similar result was first proven by Feige~\cite{feige06} for any $(2+\e)$-multiplicative factor approximation algorithm for the number of edges using only degree queries. 


\begin{thm}[Thm. 3.2 in \cite{Goldreich2008}]
  \label{thm:edge-counting}
  Let $\mA$ be an algorithm that approximates the number of edges using $Q$ consisting of neighbor, degree, and pair queries. Specifically, for any $\e > 0$, on any input graph $G = (V, E)$ with $\abs{V} = n$ and $\abs{E} = m$, $\mA$ outputs an estimate $\mhat$ satisfying $\Pr(\abs{\mhat - m} < \e / 2) \geq 2/3$. Then the expected query complexity of $\mA$ is $\Omega(n \big{/} \sqrt{\e m})$.
\end{thm}

\begin{proof}
To prove Theorem~\ref{thm:edge-counting}, we take $f = \disj$, the disjointness function (Definition~\ref{dfn:disj}). For Step~2 in the framework above, the idea is to ``hide'' edges from the algorithm by possibly including a small subgraph that nonetheless contributes a constant fraction of the edges of $G$. Starting from an arbitrary graph $G'$ with $n'$ vertices and $m'$ edges, we can accomplish this by adding a clique with at least $\e m'$ edges---a clique on $2 \sqrt{\e m'}$ vertices certainly suffices. In order to hide such a clique, we add to $G'$ an additional $n'$ vertices, partitioned into sets of size $k = n / 2 \sqrt{\e m'}$. Each set in the partition corresponds to a single bit of Alice and Bob's inputs in $\set{0, 1}^k$. In the case where Alice and Bob's inputs are disjoint, the additional vertices will be isolated. On the other hand, if Alice and Bob's sets intersect, then at least one of the partitions of the new vertices will form a clique, thereby increasing the number edges in the graph beyond $(1 + \e)m'$. Thus, the output of any algorithm that approximates the number of edges in the 
new graph can be used to compute $\disj$.

Formally, let $G' = (V', E')$ be an arbitrary fixed graph with $n' = \abs{V'}$ and $m' = \abs{E'}$. Let $V = V' \cup W$, where $W = [n']$. Take $n = \abs{V} = 2 n'$. We partition $W$ such that $W = W_1 \cup \cdots \cup W_k$ where $k = n' / 2 \sqrt{\e m'}$, and $W_i = \set{(i - 1)k + 1, \ldots, k i}$. We define $\calE : \set{0, 1}^k \times \set{0, 1}^k \to \calG_n$ as follows. Given $x, y \in \set{0, 1}^k$,  all $u, v \in V$, we have $(u, v) \in E$ if and only if one of the following two conditions is satisfied:
\begin{equation}
  \label{eqn:edge-counting}
  \begin{split}
    u, v \in V' \quad\text{and}\quad (u, v) \in E'\\
    u, v \in W_i \quad\text{and}\quad i \in x \cap y.
  \end{split}
\end{equation}
That is, $W_i$ is a clique if $i \in x \cap y$ and a set of isolated vertices otherwise. See Figure~\ref{Fig:lb_edges} for an illustration.

\begin{figure}[tb!]	
	\EdgesLB
	\caption{The construction of the graph $G=\calE(x,y)$. The top subgraph is an arbitrary graph with $n'$ and $m'$ edges, and there are $n'/\sqrt{\e m}$ additional subgraphs $W_i$, each of size  $\sqrt{\e m}$. In case $x$ and $y$ intersect on the $i\th$ coordinate, the subgraph $W_i$ is a clique, and otherwise it is a set of isolated vertices.}
	\label{Fig:lb_edges}
\end{figure}

%Let $\mA$ be an algorithm for approximating the number of edges in the graph up to a $(1\pm \e/2)$ using $T$ expected queries from $Q$, and let 
Let the function $g : \calG \to \set{0, 1}$ be defined by
\[
g(G) =
\begin{cases}
  1 & \text{if } \abs{E} \leq m'\\
  0 & \text{if } \abs{E} \geq (1 + \e) m'\,.
\end{cases}
\]
%.the output of an algorithm $\mA$ for can be used to compute $g$ with probability at least $2/3$. We are now ready to formally prove Theorem~\label{thm:edge-counting}.
%\begin{proof}[Proof of Theorem~\ref{thm:edge-counting}]

  First we argue that $(\calE, g)$ is an embedding of $\disj$. To see this, note that if $\disj(x, y) = 1$, then the second condition of Equation~\eqref{eqn:edge-counting} is never satisfied. Therefore, $m = \abs{E} = \abs{E'} = m'$, so that $g(\calE(x, y)) = \disj(x, y)$. On the other hand, if $\disj(x, y) = 0$, say $x_i = y_i = 1$, then $W_i$ is a clique. Therefore, $m = \abs{E} \geq (1 + \e) m'$.

  We now bound the communication complexity required to answer queries from $Q$. 
%  Since $\calQ$ consists of neighbor, degree, and pair queries, $\abs{\calQ} = O(\log n)$. 
  For a query $q \in Q$, note that Alice and Bob can answer the query themselves (i.e., $q$ is independent of $x$ and $y$) unless $q$ is one of the following queries:
  \begin{enumerate}
  \item $\degree(v)$ with $v \in W_i\;,$
  \item $\neighbor(v, j)$ with $v \in W_i\;,$
  \item $\pair(u, v)$ with $u, v \in W_i\;$.
  \end{enumerate}
  If $q$ is any of the three queries above, then its answer can be determined using the following protocol $\Pi_q$: Alice sends $x_i$ to Bob, and Bob sends $y_i$ to Alice. If $\neg (x_i \wedge y_i)$ then Alice and Bob answer the query accordingly. Otherwise, Alice and Bob announce $x_i \wedge y_i$. 
  Thus $\abs{\Pi_q}=2$ for all $q\in Q$.
%  HERE Thus $\abs{\Pi_Q} = O(\log n)$. Thus, for all $Q \in \calQ$, $\cost_\calE(Q) = O(\log n)$. 
The theorem then follows from Theorem~\ref{thm:query-lb}. \tnote{Should we change it according to Oded's remark. He's right that this doesn't exactly fit the framework of Thm 3.3. Otherwise we can do what he calls "extend the query protocol".}
\end{proof}

\begin{rem}
  The lower bound presented above can easily be modified to allow additional restrictions on the input graph while still giving the same lower bound. For example, we may require that the input graph $G$ be connected or have small diameter. In this case, we can modify the construction by adding $O(n)$ edges, say, by connecting every vertex in the graph to some fixed vertex $v$. In this case, the argument above remains valid with minor modifications. Thus, the lower bound holds, for example, in the case where $G$ is promised to be a connected graph of diameter $2$.
\end{rem}












